Towards Unbounded Machine Unlearning

Deep machine unlearning is the problem of `removing' from a trained neural network a subset of its training set. This problem is very timely and has many applications, including the key tasks of removing biases (RB), resolving confusion (RC) (caused by mislabelled data in trained models), as well as allowing users to exercise their `right to be forgotten' to protect User Privacy (UP). This paper is the first, to our knowledge, to study unlearning for different applications (RB, RC, UP), with the view that each has its own desiderata, definitions for `forgetting' and associated metrics for forget quality. For UP, we propose a novel adaptation of a strong Membership Inference Attack for unlearning. We also propose SCRUB, a novel unlearning algorithm, which is the only method that is consistently a top performer for forget quality across the different application-dependent metrics for RB, RC, and UP. At the same time, SCRUB is also consistently a top performer on metrics that measure model utility (i.e. accuracy on retained data and generalization), and is more efficient than previous work. The above are substantiated through a comprehensive empirical evaluation against previous state-of-the-art.

==> figures_tex/combined_spiders.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[scale=0.2]{sections/figures/spiders/cifar6_spider.png}
         \caption{CIFAR-6 (forget 50-67\%).}
         \label{fig:cifar6-spider}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[scale=0.2]{sections/figures/spiders/lacuna6_spider.png}
         \caption{Lacuna-6 (forget 50-67\%).}
         \label{fig:lacuna6-spider}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[scale=0.2]{sections/figures/spiders/cifar5_spider.png}
         \caption{CIFAR-5 (forget 5\%).}
         \label{fig:cifar5-spider}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[scale=0.2]{sections/figures/spiders/lacuna5_spider.png}
         \caption{Lacuna-5 (forget 5\%).}
         \label{fig:lacuna5-spider}
     \end{subfigure}
     \caption{Small scale setting.
    %  In the setting of large forget sets, SCRUBS is the only method that achieves forgetting without sacrificing performance. Notice that Fisher is also sometimes able to forget (especially on Lacuna-6) but its test and retain accuracy is degraded as a result of unlearning.
     }
    \label{fig:large_forget_set_spiders}
\end{figure}

==> figures_tex/figure_of_counts.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[scale=0.22]{sections/figures/counts/small_scale_forget_counts.png}
         \caption{Small scale (4 settings).}
        %  \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[scale=0.22]{sections/figures/counts/large_scale_forget_counts.png}
         \caption{Large scale (8 settings).}
        %  \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[scale=0.22]{sections/figures/counts/large_forget_set_forget_counts.png}
         \caption{Large forget sets (12 settings).}
        %  \label{fig:five over x}
     \end{subfigure}
        \caption{The number of times that each method was (one of the) top performer(s) in terms of the forget error, across all settings (architectures, datasets, selective vs class forgetting, forget set size, etc.). We consider a model a top-performer if its 95\% confidence interval overlaps with that of the best mean. Small scale counts are over \{ResNet, All-CNN\} x \{CIFAR, Lacuna\} (4 total), large scale additionally x \{class, selective\} (8 total), and large forget set additionally x \{class-50\%, class-67\%, selective-50\%\} (12 total). \textbf{SCRUBS is the most consistent in terms of its ability to unlearn}.}
        \label{fig:forget_counts}
\end{figure*}

==> figures_tex/large_scale_spider.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[scale=0.22]{sections/figures/spiders/cifar10_class_spider.png}
         \caption{CIFAR-10 class unlearning.}
         \label{fig:cifar10-class-spider}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[scale=0.22]{sections/figures/spiders/cifar10_selective_spider.png}
         \caption{CIFAR-10 selective unlearning.}
         \label{fig:cifar10-selective-spider}
     \end{subfigure}
     \caption{In the \textbf{large-scale setting}, SCRUBS is the only top-performer across settings. Selective forgetting is much harder for all, but especially for EU-k and Fisher. Scale-up is multiplied by 10 for visualization purposes. Each point represents the average across ResNet and All-CNN variants. On both subplots, CF-k and Finetuning perform similarly (they perform poorly) so their lines occlude one another. For reference, the data lives in Tables \ref{tab:large_scale_class_resnet} and \ref{tab:large_scale_class_allcnn} (left) and Tables \ref{tab:large_scale_selective_resnet} and \ref{tab:large_scale_selective_allcnn} (right).}
    \label{fig:large_scale_spiders}
\end{figure*}


==> figures_tex/small_scale_spider.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
        %  \includegraphics[scale=0.25]{sections/figures/spiders/cifar5_spider_WithBadT.png}
        \includegraphics[scale=0.25]{sections/figures/spiders/cifar5_spider.png}
         \caption{CIFAR-5.}
         \label{fig:cifar5-spider}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
        %  \includegraphics[scale=0.25]{sections/figures/spiders/lacuna5_spider_WithBadT.png}
        \includegraphics[scale=0.25]{sections/figures/spiders/lacuna5_spider.png}
         \caption{Lacuna-5.}
         \label{fig:lacuna5-spider}
     \end{subfigure}
     \caption{In the \textbf{small scale setting, selective unlearning}, SCRUBS is the only top-performer across settings. Each point represents the average across ResNet and All-CNN. On the left, CF-k and Finetuning perform similarly (they perform poorly) so their lines occlude one another, and the same is true of NTK, CF-k and EU-k on the right. For reference, this data lives in Tables \ref{tab:small_scale_resnet} and \ref{tab:small_scale_allcnn}.}
    \label{fig:small_scale_spiders}
\end{figure*}

==> mia_evaluation_old.tex <==
\input{tables/mia_main_paper}
\input{figures_tex/mia_main}

Next, we consider a set of metrics targeting a privacy-critical application, for instance deletion of user data upon their request to exercise their right-to-be-forgotten. In this case, we use a Membership Inference Attack (MIA) as the metric, inspired by \citet{shokri2017membership}. At a high-level, the goal is that, after applying unlearning, the model treats examples that were in the forget set similarly as those that were truly never seen, thus preventing an `attacker' from inferring which examples were in its original training set.

Returning to our previous notation, 
%let $w^u$ denote the weights of the model after an unlearning algorithm was applied on them, $f$ denote a neural network (e.g. a deep classifier in the settings we consider), and
let $l(f(x; w^u), y)$ denote the cross-entropy loss of the unlearned model (a deep network $f$ with weights $w^u$) on example $x$ with label $y$. We abbreviate this as $l(x, y)$ from now on; dropping the dependence on $f$ and $w^u$.

The attacker is a binary classifier that takes as input loss values, coming from either the forget set $\mathcal{D}_f$ or a held-out test set $\mathcal{D}_t$, and predicts whether the example whose loss value was presented was in the training set of the original model. We train this attacker via supervised learning on a class-balanced labelled training set for this binary problem: $\mathcal{D}_{train}^b = \{ (l(x_i, y_i), y_i^b) \}$ where each $x_i$ is an example coming either from $D_f$ or $D_t$, and its binary label $y_i^b$ is defined as being 0, if $x_i \in \mathcal{D}_t$ and 1 if $x_i \in \mathcal{D}_f$. Once the binary classifier attacker is trained, we use it to make predictions for a held-out evaluation set of the binary problem: $\mathcal{D}_{eval}^b = \{ (l(x_i, y_i), y_i^b) \}$ that is also balanced between examples coming from $\mathcal{D}_f$ and $\mathcal{D}_t$, but is disjoint from $\mathcal{D}_{train}^b$. We provide full details in the Appendix.

The attacker succeeds if it achieves high accuracy on $\mathcal{D}_{eval}^b$, meaning that it can tell apart examples that were part of the original training set from those that weren't, which marks a defeat for the unlearning model in terms of this metric, since it has `left traces behind' (in this case, in terms of loss values) and leaks information about membership in the forget set. We consider that an optimal defense against this MIA corresponds to a 50\% attack accuracy; that is, no better than randomly guessing whether an example had been trained on. In principle, the Retrain oracle should defend optimally: it in fact did not train on the forget set, so the forget and test sets are simply two different held-out sets for this model whose loss values should generally be indistinguishable from each other if these sets are identically-distributed.

We present our MIA results in Table \ref{tab:mia_main_paper} for CIFAR-10 (and more detailed results in the Appendix).
%, and additional results in Tables \ref{tab:mia_allcnn_cifar_selective}, \ref{tab:mia_allcnn_cifar_class}, \ref{tab:mia_resnet_cifar_selective}, \ref{tab:mia_resnet_cifar_class}, \ref{tab:mia_allcnn_lacuna_selective}, \ref{tab:mia_allcnn_lacuna_class}, \ref{tab:mia_resnet_lacuna_selective}, \ref{tab:mia_resnet_lacuna_class} in the Appendix. 
We make the following observations: first, SCRUB, especially when equipped with its rewinding procedure, is a strong performer in terms of MIA. EU-k can also perform strongly in this metric, though not as consistently. Unsurprisingly, the original model performs poorly in this regard: it has not performed any unlearning operation, leaving the losses of the examples in the forget set to be very low (as low as the ones in the retain set), and thus easily distinguishable from the certainly-higher test set losses. We also observe that Finetune, NegGrad and CF-k all perform poorly. Between CF-k and EU-k, it is expected that the latter is stronger in this metric, as it can be viewed as an approximation of the Retrain oracle.

We also observe from Table \ref{tab:mia_main_paper} that rewinding was only triggered once, for \textit{selective} unlearning. In both selective and class unlearning, the forget set contains examples coming from the same class, but in the former, it doesn't contain \textit{all} examples of that class; the rest are in the retain set. Thus, we indeed expect that rewinding would be more useful for selective unlearning: the smaller the portion of a class in the forget set, the larger the remainder of that class in the retain set and consequently, the better we expect the model to generalize on held-out examples of that class (lower error), making it in turn more likely to need to rewind, in order to also lower the forget set error commensurately. In Figure \ref{fig:mia} we plot results for different variants of selective unlearning, with different number of examples in the forget set (from the same class) and indeed find that for smaller numbers, rewinding is triggered. Our take-away is that, when needed, rewinding can substantially improve SCRUB's MIA results.

==> tables/large_scale.tex <==
% class unlearning
% \begin{table}[] 
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c | c c | c c | c c | c c | c c | c c |}
%     \toprule
% & \multicolumn{6}{c|}{CIFAR-10} & \multicolumn{6}{c|}{Lacuna-10} \\
% \multirow{2}{*}{Model}  & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} \\
% &mean&std&mean&std&mean&std &mean&std&mean&std&mean&std \\
% \midrule
% Retrain & 14.7 & 0.2 & 0.0 & 0.0 & 100.0 & 0.0 & 2.9 & 0.3 & 0.0 & 0.0 & 99.8 & 0.6 \\
% \midrule
% Original & 16.6 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 3.1 & 0.3 & 0.0 & 0.0 & 0.0 & 0.0 \\
% Finetune &  16.4 & 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 3.0 & 0.4 & 0.0 & 0.0 & 0.0 & 0.0 \\
% Fisher & 26.4 & 1.4 & 2.5 & 0.8 & 100.0 & 0.0 & 3.3 & 0.5 & 0.0 & 0.0 & 100.0 & 0.0 \\
% NegGrad & 17.8	&1.5&	1.7&	2.6&	91.3&	7.7 & 3.4&	0.2&	0.0&	0.0&	14.9&	1.8\\
% CF-k & 15.3&	0.1&	0.0&	0.0&	0.0&	0.0 & 2.9&	0.2&	0.0&	0.0&	0.0	&0.0\\
% EU-k & 18.7	&0.4&	0.0&	0.0&	98.8&	0.2 &	3.2&	0.2&	0.0&	0.0&	4.1&	0.8\\
% SCRUBS & 15.7 & 0.2 & 0.5 & 0.0 & 100.0 & 0.0 & 3.7 & 0.4 & 0.3 & 0.2 & 100.0 & 0.0\\
% \midrule
%     \end{tabular}
%     }
%     \caption{
%     \textbf{Large-scale} results with ResNet on class forgetting.
%     }
%     \label{tab:large_resnet_class}
% \end{table}







% selective unlearning
\begin{table}[] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c | c c | c c | c c | c c | c c | c c |}
    \toprule
& \multicolumn{6}{c|}{CIFAR-10} & \multicolumn{6}{c|}{Lacuna-10} \\
\multirow{2}{*}{Model}  & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} \\
&mean&std&mean&std&mean&std &mean&std&mean&std&mean&std \\
\midrule
Retrain & \textbf{17.4} & 0.1 & \textbf{0.0} & 0.0 & 29.7 & 3.2 & \textbf{2.7} & 0.2 & \textbf{0.0} & 0.0 & 1.0 & 1.0\\
\midrule
Original & \textbf{17.4} & 0.1 & \textbf{0.0} & 0.0 & 0.0 & 0.0  & \textbf{2.7} & 0.2 & \textbf{0.0} & 0.0 & 0.0 & 0.0\\
Finetune & \textbf{17.4} & 0.1 & \textbf{0.0} & 0.0 & 0.0 & 0.0 & \textbf{2.6} & 0.1 & \textbf{0.0} & 0.0 & 0.0 & 0.0\\
Fisher & 21.2 & 0.3 & 2.9 & 0.5 & 3.0 & 2.7  & 3.1 & 0.4 & \textbf{0.0} & 0.0 & 0.0 & 0.0\\
NegGrad & 22.7 &0.6 &4.1&	0.5&	53.7&	6.8 & 4.7 &	0.2&	0.9&	0.1	&\textbf{13.0}&	1.0 \\
CF-k & \textbf{17.4}&	0.1	&\textbf{0.0}&	0.0&	0.0&	0.0 &\textbf{2.7}&	0.2&	\textbf{0.0}&	0.0&	0.0&	0.0\\
EU-k & 21.8&	0.2 &	\textbf{0.4}&	0.6&	23.7&	3.5 & 2.9&	0.1&	\textbf{0.0}&	0.0&	0.0&	0.0\\
SCRUBS & 18.0 & 0.2 & \textbf{0.0} & 0.0 & \textbf{70.3} & 4.2 & 3.0 & 0.0 & \textbf{0.0} & 0.0 & 4.7 & 3.1\\
\midrule
    \end{tabular}
    }
    \caption{
    \textbf{Large-scale} results with ResNet on selective forgetting. SCRUBS is the only method that increases the forget error on both datasets without sacrificing retain error and minimal test error degradation.
    %Among the methods that are able to achieve higher forget error on each dataset, SCRUBS leads to the smallest performance degradation. 
    %Notably, NegGrad is able to forget (though only on Lacuna-10), but in doing so degrades model performance significantly.
    }
    \label{tab:large_resnet_selective}
\end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c | c c | c c | c c | c c }
%     \toprule
% \multirow{2}{*}{model}  & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} & \multicolumn{2}{c}{RLT ($\uparrow$)}\\
% &mean&std&mean&std&mean&std&mean&std \\
% \midrule
% retrain & 2.7 & 0.2 & 0.0 & 0.0 & 1.0 & 1.0 & 100.0 & 0.0 \\
% \midrule
% original & 2.73 & 0.15 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 \\
% finetune & 2.63 & 0.12 & 0.0 & 0.0 & 0.0 & 0.0 & 38.67 & 23.63 \\
% Fisher & 3.1 & 0.35 & 0.0 & 0.0 & 0.0 & 0.0 & 100.0 & 0.0 \\
% SCRUBS & 3.0 & 0.0 & 0.0 & 0.0 & 4.67 & 3.06 & 61.0 & 43.55 \\
% NegGrad & 4.70&	0.17&	0.88&	0.12	&13.00&	1.00&	90.67&	14.43 \\
% CF-k&2.70&	0.20&	0.00&	0.00&	0.00&	0.00&	1.00&	0.00 \\
% EU-k&2.90&	0.10&	0.01&	0.02&	0.00&	0.00&	100.00	&0.00 \\
% \midrule
%     \end{tabular}
%     \caption{
%     Large scale results on Lacuna-10 with resnet, forgetting 100 samples of class 5. SCRUBS significantly outperforms Fisher in terms of forget error, and it comparable with it otherwise.
%     % readouts for lacuna10 dataset, resnet model, forget  100 samples of class 5
%     }
%     \label{tab:large_lacuna10_resnet_selective}
% \end{table}



% speedups
\begin{table}[] 
    \centering
    \begin{tabular}{c | c c | c c | c c | c c | }
    \toprule
& \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{Lacuna-10} \\
\multirow{2}{*}{Model}  & \multicolumn{2}{c|}{ResNet} & \multicolumn{2}{c|}{All-CNN} & \multicolumn{2}{c|}{ResNet} & \multicolumn{2}{c|}{All-CNN} \\
&all&selective&all&selective&all&selective&all&selective \\

\midrule
Finetune & 3.8 & 3.09 & 3.33 & 3.03 & 1.7 & 2.03 & 2.16 & 2.00 \\
Fisher & 0.08 & 0.07 & 0.16 & 0.14 & 0.08 & 0.07 & 0.16 & 0.15 \\
NegGrad & 3.4 & 2.96 & 2.30 & 2.97 & 1.66 & 1.5 & 2.41 & 2.27 \\
CF-k & 3.55 & 3.17 & 3.37 & 2.91 & 3.42 & 3.20 & 3.27 & 3.11 \\
EU-k & 1.41 & 1.26  & 1.34 & 1.20 & 1.39 & 1.28 & 1.32 & 1.26 \\
SCRUBS & 7.84 & 7.41 & 6.36 & 5.33 & 2.17 & 1.95 & 2.81 & 2.48 \\
\midrule
    \end{tabular}
    
    \caption{
    \textbf{Large-scale} speedups
    }
    \label{tab:speedup}
\end{table}

==> tables/small_scale.tex <==
\begin{table}[] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c | c c | c c | c c | c c | c c | c c |}
    \toprule
& \multicolumn{6}{c|}{CIFAR-5} & \multicolumn{6}{c|}{Lacuna-5} \\
\multirow{2}{*}{Model}  & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} \\
&mean&std&mean&std&mean&std &mean&std&mean&std&mean&std \\
\midrule
Retrain & \textbf{24.9} & 2.5 & \textbf{0.0} & 0.0 & 28.8 & 5.9 & 5.8 & 0.4 & \textbf{0.0} & 0.0 & 4.8 & 3.4\\
\midrule
Original & \textbf{24.2} & 2.6 & \textbf{0.0} & 0.0 & 0.0 & 0.0 & \textbf{5.7} & 0.4 & \textbf{0.0}& 0.0 & 0.0 & 0.0 \\
Finetune & \textbf{24.3} & 2.4 & \textbf{0.0} & 0.0 & 0.0 & 0.0 & \textbf{5.6} & 0.3 & \textbf{0.0} & 0.0 & 0.0 & 0.0 \\
Fisher & 31.6 & 3.4 & 14.0 & 6.0 & 4.8 & 5.2 & 14.0 & 3.6 & 6.7 & 3.3 & 6.4 & 8.3 \\
NTK & \textbf{24.4} & 2.6 & \textbf{0.0} & 0.0 & 22.4 & 9.2 & \textbf{5.6} & 0.5 & \textbf{0.0} & 0.0 & 0.0 & 0.0 \\
NegGrad & \textbf{25.5}	&1.1 & \textbf{0.0} & 0.0 &	\textbf{41.3}&	6.1 & \textbf{6.1}&	0.7& \textbf{0.0}&	0.0&	1.3&	2.3\\
CF-k& \textbf{22.6}&	1.9&	\textbf{0.0}&	0.0&	0.0&	0.0 & \textbf{5.8}&	0.4&	\textbf{0.0}&	0.0&	0.0&	0.0\\
EU-k& \textbf{23.5}&	1.1&	\textbf{0.0}&	0.0&	10.7&	2.3 & \textbf{5.9}&	0.6&	\textbf{0.0}&	0.0&	0.0&	0.0\\
SCRUBS & \textbf{24.2} & 1.6 & \textbf{0.0} & 0.0 & \textbf{40.8} & 1.8 & \textbf{6.2} & 0.73 & \textbf{0.0} & 0.0 & \textbf{24.8} & 5.2\\
\midrule
    \end{tabular}
    }
    \caption{
    \textbf{Small-scale} results with ResNet. SCRUBS is the only method that effectively forgets on both datasets, without hurting the retain and test performance. 
    %Notably, Fisher leads to degrading model performance significantly, while NTK in one dataset fails to forget.
    %does not hurt test nor retain error, while having high forget error as desired. In contrast, Fisher compromises performance on the test and retain sets.
    % readouts for small-cifar5 dataset, small-resnet model, forget 25 samples of class 0
    }
    \label{tab:small_resnet}
\end{table}

% \begin{table}[] 
%     \centering
%     \begin{tabular}{c | c c | c c | c c | c c }
%     \toprule
% \multirow{2}{*}{model}  & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} & \multicolumn{2}{c}{RLT ($\uparrow$)}\\
% &mean&std&mean&std&mean&std&mean&std \\
% \midrule
% retrain & 24.92 & 2.54 & 0.0 & 0.0 & 28.8 & 5.93 & 72.6 & 2.7 \\
% \midrule
% original & 24.2 & 2.63 & 0.0 & 0.0 & 0.0 & 0.0 & 1.8 & 1.3 \\
% finetune & 24.32 & 2.4 & 0.0 & 0.0 & 0.0 & 0.0 & 2.2 & 0.84 \\
% Fisher & 31.64 & 3.42 & 13.98 & 6.05 & 4.8 & 5.22 & 1.8 & 1.3 \\
% NTK & 24.36 & 2.61 & 0.0 & 0.0 & 22.4 & 9.21 & 76.8 & 8.58 \\
% SCRUBS & 24.16 & 1.64 & 0.0 & 0.0 & 40.8 & 1.79 & 42.8 & 7.85 \\

% \midrule
%     \end{tabular}
%     \caption{
%     Small scale results on CIFAR-5 with resnet. SCRUBS performs no worse than NTK and outperfoms all other baselines significantly (notably, Fisher causes high retain and test error).
%     %does not hurt test nor retain error, while having high forget error as desired. In contrast, Fisher compromises performance on the test and retain sets.
%     % readouts for small-cifar5 dataset, small-resnet model, forget 25 samples of class 0
%     }
%     \label{tab:small_cifar5_resnet}
% \end{table}


% \begin{table}[] 
%     \centering
%     \begin{tabular}{c | c c | c c | c c | c c }
%     \toprule
% \multirow{2}{*}{model}  & \multicolumn{2}{c|}{Test error ($\downarrow$)} & \multicolumn{2}{c|}{Retain error ($\downarrow$)} & \multicolumn{2}{c|}{Forget error ($\uparrow$)} & \multicolumn{2}{c}{RLT ($\uparrow$)}\\
% &mean&std&mean&std&mean&std&mean&std \\
% \midrule
% retrain & 5.8 & 0.37 & 0.0 & 0.0 & 4.8 & 3.35 & 56.6 & 6.19 \\
% \midrule
% original & 5.72 & 0.39 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 \\
% finetune & 5.64 & 0.33 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 \\
% Fisher & 14.04 & 3.62 & 6.74 & 3.32 & 6.4 & 8.29 & 31.4 & 16.74 \\
% NTK & 5.6 & 0.51 & 0.0 & 0.0 & 0.0 & 0.0 & 16.2 & 8.79 \\
% SCRUBS & 6.2 & 0.73 & 0.0 & 0.0 & 24.8 & 5.22 & 35.2 & 8.81 \\
% NegGrad & 6.07&	0.70&	0.00&	0.00&	1.33&	2.31&	10.00&	3.00 \\
% CF-k&5.80&	0.35&	0.00&	0.00&	0.00&	0.00&	1.00&	0.00\\
% EU-k&5.93&	0.58&	0.00&	0.00&	0.00&	0.00&	92.00&	11.36\\
% \midrule
%     \end{tabular}
%     \caption{
%     Small scale results on Lacuna-5 with resnet. SCRUBS performs no worse than NTK on retain and test error, while it exhibits much better forget error (NTK is very poor in this metric) and outperfoms all other baselines significantly.
%     % readouts for small-lacuna5 dataset, small resnet model, forget 25 samples of class 0
%     }
%     \label{tab:small_lacuna5_resnet}
% \end{table}
